Using Knowledge Units of Programming Languages to Recommend Reviewers for Pull Requests: An Empirical Study

Code review is a key element of quality assurance in software development. Determining the right reviewer for a given code change requires understanding the characteristics of the changed code, identifying the skills of each potential reviewer (expertise profile), and finding a good match between the two. To facilitate this task, we design a code reviewer recommender that operates on the knowledge units (KUs) of a programming language. We define a KU as a cohesive set of key capabilities that are offered by one or more building blocks of a given programming language. We operationalize our KUs using certification exams for the Java programming language. We detect KUs from 10 actively maintained Java projects from GitHub, spanning 290K commits and 65K pull requests (PRs). Next, we generate developer expertise profiles based on the detected KUs. Finally, these KU-based expertise profiles are used to build a code reviewer recommender (KUREC). In RQ1, we observe that KUREC performs as well as the top-performing baseline recommender (RF). From a practical standpoint, we highlight that KUREC's performance is more stable (lower interquartile range) than that of RF, thus making it more consistent and potentially more trustworthy. Next, in RQ2 we design three new recommenders by combining KUREC with our baseline recommenders. These new combined recommenders outperform both KUREC and the individual baselines. Finally, in RQ3 we evaluate how reasonable the recommendations from KUREC and the combined recommenders are when those deviate from the ground truth. Taking together the results from all RQs, we conclude that KUREC and one of the combined recommenders (AD_FREQ) are overall superior to the baseline recommenders that we studied. Future work in the area should thus (i) consider KU-based recommenders as baselines and (ii) experiment with combined recommenders.

==> emse-template/setup.tex <==
% ------------- Packages Used --------------------------------------------------
% They help us to produce a better looking document ;-)
% ------------------------------------------------------------------------------

% Comment the following line before compiling the final version
%\synctex
\RequirePackage{fix-cm}

\usepackage{caption}
\usepackage{multirow}
\usepackage{balance}
\usepackage{graphicx}
\usepackage{alltt}
\usepackage{relsize}
%\usepackage{xspace}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{paralist}
\usepackage{pbox}
%\usepackage{cleveref}
\usepackage[most]{tcolorbox}
\newcommand{\tabitem}{~~\llap{\textbullet}~~}

\usepackage{array}
\usepackage{amsmath}
\usepackage{multirow}
%\usepackage{array}
\usepackage{verbatim}
%\usepackage[table]{xcolor}
\usepackage{rotating}
%\usepackage{subcaption}
%\usepackage{subfigure}
\usepackage[tight,footnotesize]{subfigure}

%\usepackage{capt-of}
%\usepackage{pifont}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage[latin1]{inputenc}
%\usepackage{times}
%\usepackage{colortbl}
\usepackage{boxedminipage}
\usepackage{float}
\usepackage{cite}
\usepackage{fancyvrb}



\usepackage{balance}

\usepackage{fancybox}%for \hypobox
\usepackage{listings}
\usepackage{array}
\usepackage{afterpage}
\usepackage{pdflscape}
\usepackage{lscape}
\usepackage{rotating}

\usepackage[T1,hyphens]{url}
%\usepackage[colorlinks,urlcolor=blue]{hyperref}


%\hypersetup{
%	colorlinks=true,
%	linkcolor=blue,
%	filecolor=blue,      
%	urlcolor=blue,
%	citecolor=blue,
%}
%\urlstyle{same}

\usepackage{textcomp}
%\usepackage{latexsym}
%\usepackage{amssymb}
%\usepackage{stmaryrd}
%\usepackage{euscript}
%\usepackage{wasysym}
%\usepackage{pifont}
%\usepackage{manfnt}
%\usepackage{undertilde}
%\usepackage{ifsym}
%\usepackage{tipa}
%\usepackage{txfonts}
%\usepackage{skak}
%\usepackage{skull}
%\usepackage{eurosym}
%\usepackage{yfonts}
%\usepackage{mathdots}
%\usepackage{trsym}
%\usepackage{upgreek}
%\usepackage{chemarr}
%\usepackage{accents}
%\usepackage{nicefrac}
%\usepackage{bm}


%\usepackage{pdfsync}

%   ACM Style
%\usepackage{lcsect}
% ------------------------------------------------------------------------------






% ------------ Color Definitions -----------------------------------------------
% Whatever colors we need
% ------------------------------------------------------------------------------
\definecolor{mygray}{rgb}{0.7,0.7,0.7}
% ------------------------------------------------------------------------------






% ---------- Special commands for annotating the paper's text ------------------
\let\mymarginpar\marginparm
\marginparwidth=1cm
\marginparsep=5pt
\newcommand{\todo}[1]{\textcolor{red}{\textbf{[[#1]]}}}
\def\TODO#1{\noindent\colorbox{yellow}{\bf \textcolor{red}{TODO: #1}}}
\newcommand{\hint}[1]{\textcolor{blue}{\textbf{#1}}}
\def\fig#1{Figure~\ref{#1}}
\def\tab#1{Table~\ref{#1}}
\def\eqn#1{Equation~\ref{#1}}
\def\sec#1{Section~\ref{#1}}

\pagenumbering{arabic}
\newcommand{\reviewer}[1]{\textcolor{DeepPink1}{{\it [Reviewer says: #1]}}}
\newcommand{\safwat}[1]{\textcolor{red}{{\it [Safwat says: #1]}}}
\newcommand{\ian}[1]{\textcolor{blue}{{\it [Ian says: #1]}}}
\newcommand{\nic}[1]{\textcolor{WildStrawberry}{{\it [Nico says: #1]}}}
\newcommand{\ahmed}[1]{\textcolor{orange}{{\it [Ahmed says: #1]}}}
\newcommand{\ahsan}[1]{\textcolor{blue}{{\it \textbf{[Ahsan says: #1]}}}}
\newcommand{\fix}[1]{\textcolor{blue}{{\it \textbf{[Fix: #1]}}}}
\newcommand{\cp}[1]{\textcolor{red}{{\it [Cor-Paul says: #1]}}}
\newcommand{\kla}[1]{\textcolor{red}{{\it [Kla says: #1]}}}

\newcommand{\myfoot}[1]{\footnote{\scriptsize #1}}
\newcommand{\myurl}[1]{\myfoot{\url{#1}}}
\newcommand{\Ra}{{$\Rightarrow$}}
\newcommand{\ra}{{$\rightarrow$}}
\newcommand{\La}{{$\Leftarrow$}}
\newcommand{\la}{{$\leftarrow$}}
\newcommand{\lra}{{$\leftrightarrow$}}
\newcommand{\LRa}{{$\Leftrightarrow$}}
%\newcommand{\todo}{\bram{todo}}

\newenvironment{myindentpar}[1]%
{\begin{list}{}%
         {\setlength{\leftmargin}{#1}}%
         \item[]%
}
{\end{list}}

% \AtBeginDocument{%
%    \renewcommand{\figurename}{Figure}%
%    \newcommand{\subfigureautorefname}{\figureautorefname}%for using subfig
% %   \renewcommand{\tablename}{TABLE}%
%    \renewcommand{\tablename}{Table}%
%    \renewcommand{\subsectionautorefname}{Section}%
%    \renewcommand{\sectionautorefname}{Section}%
% }

% Hypothesis box	
% ------------------------------------------------------------------------------	
\newcommand{\hypobox}[1]{\begin{center}%	
	\noindent\thicklines\setlength{\fboxsep}{7pt}%	
	\cornersize{0}\Ovalbox{\begin{minipage}{3.1in}%	
	\vspace{-0.1cm}
	\textit{#1}
	\vspace{-0.1cm}
	\end{minipage}} \end{center}}	
% ------------------------------------------------------------------------------




% ------------------------- SYMBOLS OF SELF NAMES OFTEN USED -------------------
\newcommand{\APACHE}{{\small APACHE}\xspace}
\newcommand{\BUGZILLA}{{\small BUGZILLA}\xspace}
\newcommand{\ECLIPSE}{{\small ECLIPSE}\xspace}
\newcommand{\ASPECTJ}{{\small ASPECTJ}\xspace}
\newcommand{\JDT}{{\small JDT}\xspace}
\newcommand{\GNU}{{\small GNU}\xspace}
\newcommand{\MOZILLA}{{\small MOZILLA}\xspace}
\newcommand{\THUNDERBIRD}{{\small THUNDERBIRD}\xspace}
\newcommand{\JAVA}{{\small Java}\xspace}
\newcommand{\GNOME}{{\small GNOME}\xspace}
\newcommand{\PG}{{\small PostgreSQL}\xspace}
\newcommand{\SIM}{{\small SimScan}\xspace}


\newcommand{\NEGDIFF}{{\emph{Neg}$_{\text{\emph{Diff}}}$}}



% Anything else, e.g., \NAME{MICROSOFT}
\newcommand{\NAME}[1]{{\small #1}\xspace}
% ------------------------------------------------------------------------------




% ----------------------- Computer Science lol ---------------------------------
% Variable, function, and program names
% ------------------------------------------------------------------------------
\newcommand{\smalltt}[1]{\ifmmode{\mbox{\smaller\texttt{#1}}}\else{\smaller\tt #1}\fi}
\newcommand{\code}[1]{\smalltt{#1}}
\newcommand{\var}[1]{\code{#1}}
\newcommand{\func}[1]{\code{#1}}
\newcommand{\proc}[1]{\code{#1}}
\newcommand{\prog}[1]{\code{#1}}
\newcommand{\type}[1]{\code{#1}}
\newcommand{\progpt}[1]{\code{#1}}

\newcommand{\mypar}[1]{\vspace{.1cm}\noindent \textbf{#1}}
\newcommand{\myxpar}[1]{\vspace{.1cm}\noindent \textbf{#1}\newline}
% ------------------------------------------------------------------------------





% ----------- Things to remember -----------------------------------------------
\newenvironment{mynote}%
{ \medskip
  \noindent
  \let\emph=\textbf
  \begin{boxedminipage}{\columnwidth}\em}%
{ \end{boxedminipage}}
% ------------------------------------------------------------------------------






% -------------------- Use bars ------------------------------------------------
% These macros are for advanced presentation of results by shaded bars only!
% © Tom Zimmermann, 2008
% ------------------------------------------------------------------------------
\newdimen\qdx
\newdimen\qda
\newdimen\qdb
\def\rrrr#1#2#3#4{\newdimen\qd\qd=#4 % length of bar for 1.0
\qdx=\qd\multiply\qdx by 5\divide\qdx by 4
\qda=\qd
\qdb=\qd
\multiply\qda by #1\divide\qda by #3\multiply\qdb by #2\divide\qdb by #3\advance\qdb by -\qda
    \leavevmode\hbox to \qdx{\hfil\vbox{%
    \hbox{\vrule\vbox{\hrule\hbox to 1\qd
            {\vrule depth0pt height0.7ex width \qda\color{mygray}%
 \vrule depth0pt height0.7ex width \qdb\hfill}\hrule}\vrule}
    }\hfil}}
\def\rrr#1#2#3{\rrrr{#1}{#2}{#3}{0.8cm}}
% -------------------------------------------------------------------------






% ------------ Graphics Hacks --------------------------------------------------
% Use these settings if Figures tend to get their one separate pages
% ------------------------------------------------------------------------------
% \renewcommand{\topfraction}{0.85}
% \renewcommand{\textfraction}{0.1}
% \renewcommand{\floatpagefraction}{0.75}
% ------------------------------------------------------------------------------





% ------------------ Biblio Hack -----------------------------------------------
% Use these settings if the References take too much space
% ------------------------------------------------------------------------------
\let\oldthebibliography=\thebibliography
  \let\endoldthebibliography=\endthebibliography
  \renewenvironment{thebibliography}[1]{%
%	\vspace{-0.3cm}
    \begin{oldthebibliography}{#1}%
%	\vspace{-0.2cm}
       \setlength{\parskip}{0ex}%
       \setlength{\itemsep}{0ex}%
%	\bibfont
  }%
  {%
    \end{oldthebibliography}%
  }
% ------------------------------------------------------------------------------





% -------------- Floats Redefined ----------------------------------------------
% Use these settings to change the whitespace between floats and text
% ------------------------------------------------------------------------------

% \setlength\dblfloatsep{1pt}
% \setlength\floatsep{1pt}
% \setlength\textfloatsep{5pt}
% \setlength\dbltextfloatsep{5pt}

% \renewcommand\floatpagefraction{.9}
% \renewcommand\topfraction{.9}
% \renewcommand\bottomfraction{.9}
% \renewcommand\textfraction{.1}
% \setcounter{totalnumber}{50}
% \setcounter{topnumber}{50}
% \setcounter{bottomnumber}{50}
% ------------------------------------------------------------------------------



% The custom defined cell types, I needed this to make the headers centered but the remaining of the column is right or left justified.
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\usepackage{tikz}
\usetikzlibrary{shapes.geometric,calc}

\newcommand\score[2]{
	\pgfmathsetmacro\pgfxa{#1+1}
	\tikzstyle{scorestars}=[star, star points=5, star point ratio=2.25, draw,inner sep=0.15em,anchor=outer point 3]
	\begin{tikzpicture}[baseline]
	\foreach \i in {1,...,#2} {
		\pgfmathparse{(\i<=#1?"yellow":"gray")}
		\edef\starcolor{\pgfmathresult}
		\draw (\i*1em,0) node[name=star\i,scorestars,fill=\starcolor]  {};
	}
	\pgfmathparse{(#1>int(#1)?int(#1+1):0}
	\let\partstar=\pgfmathresult
	\ifnum\partstar>0
	\pgfmathsetmacro\starpart{#1-(int(#1))}
	\path [clip] ($(star\partstar.outer point 3)!(star\partstar.outer point 2)!(star\partstar.outer point 4)$) rectangle 
	($(star\partstar.outer point 2 |- star\partstar.outer point 1)!\starpart!(star\partstar.outer point 1 -| star\partstar.outer point 5)$);
	\fill (\partstar*1em,0) node[scorestars,fill=yellow]  {};
	\fi
	
	,\end{tikzpicture}
}

\newcommand{\smallnum}[1]{$^{\tiny {\textbf #1}}$}

\newcommand{\specialcell}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}

\newcommand{\specialcellLeft}[2][t]{%
	\begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}

\usepackage{threeparttable, tablefootnote}

\newtcolorbox[auto counter]{summary_RQ1}[1][]{title={\bfseries Summary of RQ1},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}

\newtcolorbox[auto counter]{summary_RQ2}[1][]{title={\bfseries Summary of RQ2},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}
	
\newtcolorbox[auto counter]{summary_RQ3}[1][]{title={\bfseries Summary of RQ3},enhanced,
	coltitle=black,
	top=0.17in,
	attach boxed title to top left=
	{xshift=1.5em,yshift=-\tcboxedtitleheight/2},
	boxed title style={size=small,colback=lightgray},#1}

==> ieee-template/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/Bios.tex <==
\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/ahsan.jpg}}]
    {\scriptsize Md Ahasanuzzaman}\scriptsize is currently a Ph.D. student in the Software Analysis and Intelligence Lab (SAIL) at Queen's University, Canada. His research interests include mining software repositories (e.g., mobile app stores), source code analysis (e.g., mobile apps, Java applications), and machine learning. His studies got published in top Software Engineering venues (e.g., TSE, EMSE, and MSR). He obtained his BSc from the University of Dhaka in Bangladesh. He has been awarded prestigious awards, such as Deans scholarship award and Prime Minister Gold Medal for his outstanding achievements in the B.Sc program. More information at: \url{https://ahasanuzzaman.com/research/}
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
	[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/gus-bw.png}}]
	{\scriptsize Gustavo A. Oliva} \scriptsize is an Adjunct Professor at the School of Computing of Queen's University in Canada. Gustavo leads the blockchain research team at the Software Analysis and Intelligence Lab (SAIL). In addition to blockchain, he also conducts empirical studies in the fields of software ecosystems (e.g., npm), software evolution, and explanaible AI. Gustavo received his MSc and PhD degrees from the University of São Paulo (USP) in Brazil under the supervision of professor Dr. Marco Aur{é}lio Gerosa. More information at: \url{https://www.gaoliva.com}
\end{IEEEbiography}

\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{figures/Bios/ahmed.jpg}}]
    {\scriptsize Ahmed E. Hassan} \scriptsize is an IEEE Fellow, an ACM SIGSOFT Influential Educator, an NSERC Steacie Fellow, the Canada Research Chair (CRC) in Software Analytics, and the NSERC/BlackBerry Software Engineering Chair at the School of Computing at Queen’s University, Canada. His research interests include mining software repositories, empirical software engineering, load testing, and log mining. He received a PhD in Computer Science from the University of Waterloo. He spearheaded the creation of the Mining Software Repositories (MSR) conference and its research community. He also serves/d on the editorial boards of IEEE Transactions on Software Engineering, Springer Journal of Empirical Software Engineering, and PeerJ Computer Science. More information at: \url{http://sail.cs.queensu.ca}
\end{IEEEbiography}

==> sections/Discussion.tex <==
\section{Discussion} \ahsan{Added this section. Please check this section Gustavo.}
\label{sec:discussion}

In this section, we conduct follow-up studies of our KUREC model. In particular, we study three important aspects of KUREC for recommending code reviewers: (1) how robust the performance of KUREC in recommending code reviewers for the PRs consisting of new files?, (2) how far the correct reviewers (the ones who actually reviewed the PRs) are ranked by KUREC for those PRs that KUREC can not recommend them correctly in top-5 recommendations?, and (3) how good are the top-k recommendations of KUREC for those PRs that KUREC can not recommend the correct reviewer in top-5 recommendations? For each of the above-mentioned studies, we compare the performance of KUREC with the performance of CHREV. Our rationale for choosing CHREV is two folds: (1) CHREV is the most advanced recommender among the baselines, and (2) the performance of the CHREV is consistent for the dataset. 


\subsection{How robust the performance of KUREC in recommending code reviewers for the PRs consisting of new files?} 
\noindent \textbf{Motivation.} The robustness of a recommender is an important aspect that build trust among users~\citep{mobasher2007toward}. Recommenders (e.g., KUREC and CHREV) learn from the files of PRs in the train dataset and generate a score to recommend reviewers for the PRs in the test dataset. However, recommenders may need to recommend reviewers for PRs consisting of files that are new (i.e., these files were never seen in the training dataset). Such cases could drastically hamper the performance of recommenders and cause an issue about trustworthiness of recommenders~\citep{mobasher2007toward}. Therefore, it is important to understand how robust the performance of a recommender in recommending reviewers for the PRs consisting of new files.


\noindent \textbf{Approach.} For this study, we need to select PRs in the test dataset that contain new files (i.e., those files are not present in the train dataset). To identify a new file of a PR in the test dataset, we compare the path of every file of the PR in the test dataset to the path of all files of PRs in the train dataset. We identify a new file of a PR if the path of the file does not match with the path of any files in the train dataset. Then, we calculate the percentage of new files for each PR in the test dataset for every studied project. Since a PR can contain multiple files, we use a threshold to select the PRs for this study. We select the PRs for this study if the percentage of new files of the PRs is above 50\%. \ahsan{any suggestion to justify the threshold? I think 50\% is a good threshold to understand how the recommender performs if more than half of the files are new.} We observe that the minimum number of the selected PRs in a project is at least 10 and the maximum number of the selected PRs in a project is 226. Finally, we use the selected PRs to test the KUREC and CHREV, and calculate the top-k accuracy for these recommenders.

\begin{table}[]
    \caption{The top-k accuracy values of recommenders for the PRs that contain new files requesting for reviewing.}
    \label{tab:further-study-new-file}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lllllll@{}}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Project}}}                      & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Recommender\\ Name\end{tabular}}}} & \multicolumn{5}{c}{\textbf{Top-k Accuracy}}                                                                                                                                  \\ \cmidrule(l){3-7} 
    \multicolumn{1}{c}{}                                                       & \multicolumn{1}{c}{}                                                                                     & \multicolumn{1}{c}{\textbf{k=1}} & \multicolumn{1}{c}{\textbf{k=2}} & \multicolumn{1}{c}{\textbf{k=3}} & \multicolumn{1}{c}{\textbf{k=4}} & \multicolumn{1}{c}{\textbf{k=5}} \\ \midrule
    \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ ActiveMQ\end{tabular}} & 
    CF                                                                                                    & 0.00                             & 0.00                            & 0.00                             & 0.00                             & 0.00                             \\ &

    RF                                                                                                    & 0.69{**}                             & 0.69{**}                            & 0.77{**}                             & 0.85{**}                             & 0.92{**}                             \\ &

    ER                                                                                                    & 0.08                             & 0.15{*}                            & 0.15{*}                             & 0.15{*}                             & 0.15{*}                             \\ &

    CHREV                                                                                                    & 0.00{*}                             & 0.08                             & 0.08                             & 0.08                             & 0.15                             \\
                                                                               & KUREC                                                                                                    & 0.31{*}                           & 0.77{**}                             & 0.77{**}                             & 0.77{**}                             & 0.77{**}                             \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Groovy\end{tabular}}   & 
    
    CF                                                                                                    & 0.40{**}                             & 0.60{**}                             & 0.70{**}                             & 0.70{**}                             & 0.70{**}                             \\&

    RF                                                                                                    & 0.60{**}                             & 1.00{**}                             & 1.00{**}                             & 1.00{**}                             & 1.00{**}                             \\&

    ER                                                                                                    & 0.40{**}                             & 0.40{*}                             & 0.40{*}                             & 0.60{*}                             & 0.60{*}                             \\&

    CHREV                                                                                                    & 0.10                             & 0.10                             & 0.10                             & 0.10                             & 0.10                             \\
                                                                               & KUREC                                                                                                    & 0.70{*}                             & 0.90{**}                             & 1.00{**}                             & 1.00{**}                             & 1.00                             \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Lucene\end{tabular}}   & 

    CF                                                                                                    & 0.50{*}                            & 0.64{*}                             & 0.68                             & 0.77                             & 0.82                             \\ &

    RF                                                                                                    & 0.50{*}                            & 0.82{*}                             & 0.82{*}                             & 0.86{*}                             & 0.86{*}                             \\ &
    
    ER                                                                                                    & 0.50                            & 0.55                             & 0.59                             & 0.64{*}                             & 0.68{*}                             \\ &

    CHREV                                                                                                    & 0.18{**}                             & 0.18                             & 0.18                             & 0.18                             & 0.23                             \\
                                                                               & KUREC                                                                                                    & 0.68{*}                             & 0.77{**}                             & 0.91{**}                             & 1.00{**}                             & 1.00{**}                             \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache \\ Hbase\end{tabular}}   & 
    
    CF                                                                                                    & 0.20                            & 0.30                             & 0.30                             & 0.30{*}                             & 0.30                             \\ &

    RF                                                                                                    & 0.28                            & 0.45                             & 0.57{*}                             & 0.57{*}                             & 0.62{**}                             \\ &

    ER                                                                                                    & 0.18{*}                            & 0.20{*}                             & 0.22{*}                             & 0.30{*}                             & 0.30                             \\ &
    
    CHREV                                                                                                    & 0.03{*}                             & 0.18                             & 0.20                             & 0.25                             & 0.25                             \\
                                                                               & KUREC                                                                                                    & 0.25{**}                             & 0.53{**}                             & 0.58{**}                             & 0.58{**}                             & 0.60{**}                             \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Hive\end{tabular}}     & 
    
    CF                                                                                                    & 0.07{**}                             & 0.10{**}                             & 0.12{**}                             & 0.15{**}                             & 0.15{**}                             \\&

    RF                                                                                                    & 0.05{**}                             & 0.22{**}                             & 0.39{**}                             & 0.51{**}                             & 0.59{**}                             \\&

    ER                                                                                                    & 0.12                             & 0.20                             & 0.20                             & 0.22                             & 0.22                             \\&
    
    CHREV                                                                                                    & 0.05                             & 0.10                             & 0.10                             & 0.12                             & 0.17                             \\
                                                                               & KUREC                                                                                                    & 0.20{**}                             & 0.29{**}                             & 0.39{**}                             & 0.46{**}                             & 0.54{**}                             \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Storm\end{tabular}}    & 
    
    CF                                                                                                    & 0.00                             & 0.00                             & 0.00                             & 0.00                             & 1.00                             \\&

    RF                                                                                                    & 0.00                             & 0.00                             & 0.33                             & 0.67{*}                             & 1.00{*}                             \\&

    ER                                                                                                    & 0.11                             & 0.11                             & 0.11                             & 0.11                             & 0.11                             \\&

    CHREV                                                                                                    & 0.22                             & 0.22                             & 0.22                             & 0.22                             & 0.22                             \\
                                                                               & KUREC                                                                                                    & 0.00                             & 0.11                             & 0.22                             & 0.56{*}                             & 0.89{**}                             \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Wicket\end{tabular}}   & 
    
    CF                                                                                                    & 0.00                             & 0.00                             & 0.20{**}                             & 0.30 {**}                            & 0.40                             \\&

    RF                                                                                                    & 1.00{**}                             & 1.00{**}                             & 1.00                             & 1.00                             & 1.00                             \\&

    ER                                                                                                    & 0.10{**}                             & 0.10{**}                             & 0.30{**}                             & 0.30{*}                             & 0.40{*}                             \\&
    
    CHREV                                                                                                    & 0.40{**}                             & 1.00{**}                             & 1.00{**}                             & 1.00{**}                             & 1.00{**}                            \\
                                                                               & KUREC                                                                                                    & 0.60{**}                             & 0.80{**}                             & 1.00{**}                             & 1.00{**}                             & 1.00{**}                             \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Elastic\\ Search\end{tabular}}  & 
    
    CF                                                                                                    & 0.15{**}                             & 0.19{*}                             & 0.23{*}                             & 0.26{*}                             & 0.27{*}                             \\&

    RF                                                                                                    & 0.02{*}                             & 0.08{*}                             & 0.12{*}                             & 0.17{*}                             & 0.19{*}                             \\&

    ER                                                                                                    & 0.18{*}                             & 0.24{*}                             & 0.26{*}                             & 0.30{*}                             & 0.31{*}                             \\&
    
    CHREV                                                                                                    & 0.12                             & 0.17                             & 0.20                             & 0.22                             & 0.24                             \\
                                                                               & KUREC                                                                                                    & 0.16{*}                             & 0.23{*}                             & 0.28{*}                             & 0.30{*}                             & 0.35{*}                             \\ \midrule \midrule
    \multirow{2}{*}{Median}                                                    & 
    CF                                                                                                    & 0.11{**}                             & 0.15{**}                             & 0.21{**}                             & 0.28{**}                             & 0.28{*}                             \\&

    RF                                                                                                    & 0.39{**}                             & 0.57{**}                             & 0.67{**}                             & 0.76{**}                             & 0.89{**}                             \\&

    ER                                                                                                    & 0.15{*}                             & 0.20{*}                             & 0.24{*}                             & 0.30{*}                             & 0.30{*}                             \\&

    CHREV                                                                                                    & 0.11                             & 0.17                             & 0.19                             & 0.20                             & 0.22                             \\
                                                                               & KUREC                                                                                                    & 0.28{**}                             & 0.65{**}                             & 0.67{**}                             & 0.67{**}                             & 0.83{**}                             \\ \bottomrule
                                                                               \multicolumn{7}{l}{\pbox{50cm}{1. The \textbf{two asterisks} (\textbf{**}) beside the top-k accuracy value denote that the}}\\
\multicolumn{7}{l}{\pbox{50cm}{\textbf{value is 20\% lower} than the top-k accuracy value of recommenders }}\\
\multicolumn{7}{l}{\pbox{50cm}{that are tested on all test dataset (i.e., Table~\ref{tab:rq3-accuracy}).}}\\

\multicolumn{7}{l}{\pbox{50cm}{2. The \textbf{single asterisk} (\textbf{*}) beside the top-k accuracy value denotes that the}}\\
\multicolumn{7}{l}{\pbox{50cm}{\textbf{value is 50\% lower} than the top-k accuracy value of recommenders}}\\
\multicolumn{7}{l}{\pbox{50cm}{that are tested on all test dataset (i.e., Table~\ref{tab:rq3-accuracy}).}} \\

\multicolumn{7}{l}{\pbox{50cm}{3. \textbf{No asterisk} beside the top-k accuracy value denotes that the}}\\
\multicolumn{7}{l}{\pbox{50cm}{\textbf{value is more than 50\% lower} than the top-k accuracy value of recommenders}}\\
\multicolumn{7}{l}{\pbox{50cm}{that are tested on all test dataset (i.e., Table~\ref{tab:rq3-accuracy}).}}
    \end{tabular}
    }
    \end{table}



    \begin{table}[]
        \caption{The percentage of PRs that the top-1 recommended reviewer of recommenders has prior experience for reviewing the changed files.}
        \label{tab:further-study-review-history}
        \centering
        \begin{tabular}{@{}lr@{}}
            \toprule
            \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Recommender\\ Name\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Percentage\\ of PRs\end{tabular}}} \\ \midrule
            CF                                                                                      & 24.1\%                                                                                   \\
            RF                                                                                      & 13.5\%                                                                                   \\
            ER                                                                                      & 57.8\%                                                                                   \\
            CHREV                                                                                   & 33.2\%                                                                                   \\
            KUREC                                                                                   & 63.3\%                                                                                   \\ \bottomrule
            \end{tabular}
        \end{table}

\noindent \textbf{Findings.} \observation{The performance of KUREC is robust, and KUREC outperforms CHREV for PRs containing new files.} Table~\ref{tab:further-study-new-file} presents the top-k accuracy values of KUREC and CHREV for the PRs containing new files. We observe that KUREC outperforms CHREV in all the studied projects across all top-k accuracy values. KUREC achieves three times more accuracy than CHREV in the top-5 recommendations (the median top-5 accuracy of KUREC is 0.83, whereas the median top-5 accuracy of CHREV is 0.22). We also observe that the performance of KUREC for PRs containing new files does not change much compared to the performance of KUREC for the entire test dataset (see Table~\ref{tab:rq3-accuracy}). The majority of the top-k accuracy values of KUREC are 20\% lower than the top-k accuracy values of KUREC that is tested on all test dataset (see values with two asterisks {(**)}). On the other hand, the top-k accuracy of CHREV is drastically impacted by the new files of PRs. The majority of the top-k accuracy values of CHREV are more than 50\% lower than the top-k accuracy values of CHREV that is tested on all test dataset (see values with no asterisk (*)). Such a result indicates that KUREC is more robust than CHREV for the PRs containing new files. 

One possible reasons for the poor performance of CHREV on PRs containing new files is that CHREV depends on the past contribution (e.g., review comments) of reviewers on the files associated with the given PR for testing. There is no past contribution for the new files of a given PR, and CHREV can not generate appropriate score for reviewers (i.e., cold start problem~\citep{lika2014facing}). On the contrary, KUREC depends on the knowledge units (KUs) of the files associated with PRs. Even though there are new files in a given PR for testing, KUREC can still generate expertise scores for developers using the KUs of the files of past PRs (PRs that are preceding to the given one for testing) that contain similar KUs of the files in the given PR. Hence, KUREC can overcome the cold start problem of recommenders and achieve a better top-k accuracy than CHREV.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
    \caption{The statistics of the ranking of the correct reviewers of KUREC and CHREV across projects.}
    \label{tab:stats-first-correct-reviewer-ranking}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}llcccccc@{}}
    \toprule
    Project                                                                    & \begin{tabular}[c]{@{}l@{}}Recommender\\ Name\end{tabular} & Min & Q1 & Median & Q3  & Max & IQR \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ ActiveMQ\end{tabular}} & CHREV                                                      & 28  & 30 & 55     & 64  & 64  & 34  \\
                                                                               & KUREC                                                      & 7   & 9  & 13     & 45  & 77  & 36  \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Hbase\end{tabular}}    & CHREV                                                      & 6   & 12 & 87     & 135 & 282 & 123 \\
                                                                               & KUREC                                                      & 6   & 10 & 19     & 24  & 66  & 14  \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Hive\end{tabular}}     & CHREV                                                      & 6   & 11 & 50     & 134 & 383 & 123 \\
                                                                               & KUREC                                                      & 6   & 8  & 13     & 25  & 67  & 17  \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Lucene\end{tabular}}   & CHREV                                                      & 8   & 95 & 187    & 278 & 282 & 183 \\
                                                                               & KUREC                                                      & 6   & 6  & 7      & 10  & 56  & 4   \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Apache\\ Storm\end{tabular}}    & CHREV                                                      & 6   & 9  & 40     & 175 & 305 & 166 \\
                                                                               & KUREC                                                      & 6   & 6  & 7      & 7   & 9   & 1   \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Elastic\\ Search\end{tabular}}  & CHREV                                                      & 6   & 8  & 65     & 206 & 400 & 198 \\
                                                                               & KUREC                                                      & 6   & 10 & 17     & 34  & 118 & 24  \\ \bottomrule
    \end{tabular}
    }
    \end{table}

\subsection{How far the correct reviewers are ranked by KUREC for those PRs that KUREC can not recommend reviewers correctly in top-5 recommendations?}

\noindent \textbf{Motivation.} Recommenders may not always recommend a  correct reviewer (i.e., the one who actually reviewed the PR) within the top-5 recommendations. Studying the recommendations of a recommender for these cases can help us understand the range of the ranking for recommending the correct reviewer in worst-case scenarios. 

\noindent \textbf{Approach.} First, we select the PRs in the test dataset that KUREC can not recommend a correct reviewer within the top-5 recommendations. Then, we identify the rank of a correct reviewer from the recommendation of KUREC for each of the selected PRs. Finally, we generate a distribution of the ranking of the correct reviewers for KUREC. Similarly, we follow the above-mentioned steps for CHREV and generate a distribution of the ranking of the correct reviewer for CHREV.  

\noindent \textbf{Findings.} \observation{The rank of the correct reviewer of KUREC is better than CHREV.} Table~\ref{tab:stats-first-correct-reviewer-ranking} presents the statistics of the rank of the correct reviewer of KUREC and CHREV for those PRs that these recommenders can not recommend the correct reviewer in top-5 recommendations. We observe that the rank of the correct reviewer of KUREC is smaller than CHREV. The median rank of the correct reviewer of KUREC is 16 across all the studied projects. The median rank of the correct reviewer of CHREV is four times to the median rank of KUREC for each of the studied projects. We also observe that the rank of KUREC is more stable than CHREV. The interquartile range of the rank of CHREV is more than five times to the interquartile range of KUREC. These results indicate that KUREC can offer consistent performance and recommend the correct reviewer in a better rank than CHREV in worst-case scenarios (i.e., PRs that recommenders can recommend the correct reviewer in top-5 recommendations).




%\begin{figure}[!ht]
%    \centering
%    \includegraphics[width=1\linewidth]{./figures/Discussion/first_correct_reviewer_rank}
%    \caption{The distribution of the ranking of correct reviewer for the PRs that the KUREC and CHREV can not identify the correct reviewer in top-5 recommendations.}
%    \label{fig:discussion-first-correct-reviewer}
%\end{figure}

\subsection{How good are the top-k recommendations of KUREC for those PRs that KUREC can not recommend the correct reviewer in top-k recommendations?}

\noindent \textbf{Motivation.} A recommender can recommend reviewers with similar expertise, although the recommended reviewer is not the correct reviewer (i.e., the reviewer who reviewed this PR) for the PR. However, these recommended reviewers could be capable in reviewing the PR and the recommendation of the reviewers could be acceptable. Therefore, we study the top recommendation of KUREC and CHREV to understand whether the recommended reviewers are capable of reviewing the files in PRs.

\noindent \textbf{Approach.} We perform the following steps for both KUREC and CHREV recommenders. 

\noindent \textit{Determining if reviewers have prior expertise in reviewing or modifying the changed files.} First, we select the PRs from the test dataset that a recommender can not recommend the correct reviewer within top-5 recommendations. We select 1,165 PRs for KUREC and 1,227 PRs for CHREV. Then, we select the top recommended reviewer (i.e., top-1 ranked reviewer) for each of the selected PRs of a recommender. To understand if the selected reviewer has expertise for reviewing the changed files in a PR \textit{P}, we check if the changed files of the PR were reviewed or modified by the reviewer. Finally, if we find the changed files of \textit{P} among the changed files of PRs and commits that are created preceding to the creation time of \textit{P}, we determine that the reviewer has expertise for reviewing the changed files in that PR \textit{P}.

\noindent \textit{Selecting a sample of PRs for manual study.} To investigate manually, we select a sample of PRs that are common in the selected PRs of KUREC and CHREV. We find that 791 PRs are common in the selected PRs of KUREC and CHREV. We manually examine a statistically representative random sample of these 791 PRs (65) to validate if the top reviewer of the recommenders has prior expertise to review the changed files.
%We search the name of the changed files of the selected PR among the changed files of PRs and commits that are created preceding to the selected PR.

\noindent \textbf{Findings.} \observation{Though the correct reviewer is not present at top-5 recommendations, the top recommended reviewer of KUREC has expertise in reviewing PRs.} We observe that the top-1 recommended reviewer of KUREC has prior experience in reviewing or modifying the changed files in 77\% of the selected PRs. This number is low for CHREV. We observe that the top-1 recommended reviewer of CHREV has prior experience in reviewing or modifying the changed files in 43\% of the selected PRs. Such a result indicates that KUREC's recommendation is reliable and better than CHREV. 

Our manual study also confirms that the top-1 recommended reviewer of KUREC has expertise and is capable of reviewing PRs. As an example, we highlight a pull request of ElasticSearch (PR\#77464)\footnote{\url{https://github.com/elastic/elasticsearch/pull/77464}} that provides fixes for a date related issue. To fix the issue, ``CanMatchPreFilterSearchPhaseTests.java'' file was modified. We find that KUREC can not recommend the correct reviewer for this PR. However, the top-1 recommended reviewer of KUREC (Jim Ferenczi\footnote{\url{https://github.com/jimczi?tab=overview\&from=2021-12-01\&to=2021-12-31}}) has experience in reviewing and modifying the file (i.e., ``CanMatchPreFilterSearchPhaseTests.java''). We find that the top-1 recommended reviewer of KUREC previously reviewed the file in PR\#65583\footnote{\url{https://github.com/elastic/elasticsearch/pull/65583/files\#r542380492}} and modified the same file in a commit\footnote{\url{https://github.com/elastic/elasticsearch/commit/2c7039}}. As such, the reviewer has knowledge about the code and is capable of reviewing the file. Such an example illustrates that KUREC's recommended reviewers are indeed capable of reviewing PRs.

\begin{footnotesize}
    \begin{mybox}{Summary}
        Follow-up Study:
        \tcblower
    	\begin{itemize}[itemsep = 3pt, label=\textbullet, wide = 0pt]
            \item KUREC's performance is robust, outperforming CHREV in recommending reviewers for PRs containing new files.
            \item The top-1 recommended reviewer of KUREC is indeed capable of reviewing PRs even though the top-1 recommended reviewer is not the correct one.
    	\end{itemize}
    \end{mybox}
\end{footnotesize}





==> sections/Findings.tex <==
\section{Findings}
\label{sec:Findings}

%We linked the RQs' findings here



\input{sections/Findings-RQ1}
\input{sections/Findings-RQ2}
\input{sections/Findings-RQ3}
